Equitable Network-Aware Decarbonization of Residential Heating at City Scale

Residential heating, primarily powered by natural gas, accounts for a significant portion of residential sector energy use and carbon emissions in many parts of the world. Hence, there is a push towards decarbonizing residential heating by transitioning to energy-efficient heat pumps powered by an increasingly greener and less carbon-intensive electric grid. However, such a transition will add additional load to the electric grid triggering infrastructure upgrades, and subsequently erode the customer base using the gas distribution network. Utilities want to guide these transition efforts to ensure a phased decommissioning of the gas network and deferred electric grid infrastructure upgrades while achieving carbon reduction goals. To facilitate such a transition, we present a network-aware optimization framework for decarbonizing residential heating at city scale with an objective to maximize carbon reduction under budgetary constraints. Our approach operates on a graph representation of the gas network topology to compute the cost of transitioning and select neighborhoods for transition. We further extend our approach to explicitly incorporate equity and ensure an equitable distribution of benefits across different socioeconomic groups. We apply our framework to a city in the New England region of the U.S., using real-world gas usage, electric usage, and grid infrastructure data. We show that our network-aware strategy achieves 55% higher carbon reductions than prior network-oblivious work under the same budget. Our equity-aware strategy achieves an equitable outcome while preserving the carbon reduction benefits of the network-aware strategy.

==> future.tex <==

\noman{Adding random text that comes to my mind. }
\noman{An additional selection criteria for removing gas pipelines can be the gas leakage factor. Old pipeline (or pipelines made of certain materials) will have high leakage factors. Utilities may be incentivized to remove leaking pipelines.}

\noman{There are two main types of gas pipelines: gas mains and gas service lines. Mains lines are of bigger diameter and many service lines originate from the main lines. Service lines connect gas meters to the main lines. There may be gas pressure regulators between the main and service lines. Utilities would prefer to remove service lines that connect to only single gas main as they do not have to worry about the gas flow in the network. These service lines at the edge of the network should be prioritized.}

\mo{these are good to mention as future work in conclusion, or if the list is long we can have a discussion section and list them as "additional practical challenges". I feel it is hard to have sufficiently accurate data to bring them into the main body of the problem. }

==> newintro.tex <==
In the United States, residential heating is responsible for roughly 50\% of total residential energy use.  Large parts of the world depend on fossil fuels such as oil, propane, or natural gas for heating homes when outdoor temperatures are low -- in the U.S., residential energy use contributes about 20\% of the total yearly greenhouse gas emissions \cite{X}.  The decarbonization of residential heating, ventilation, and air conditioning (HVAC) systems is therefore an important goal for a carbon-free future.

To address this problem, a promising method is to electrify heating systems by replacing fossil fuel-based HVAC components such as furnaces and boilers with electric heat pumps (EHPs).  

Heat pump technology has advanced significantly over the past decade, enabling drop-in, air-source units which maintain good efficiency even at temperatures as low as -15$^{\circ}$C \cite{Johnson:2021, Schoenbauer:2016}, making them appropriate for use in cold climates.  From an efficiency perspective, heat pumps use less energy compared to fossil fuel combustion to output the same amount of heat \cite{OEERE}.  Combined with the ability to source electricity from carbon-free and renewable sources, this advantage makes heat pumps a great potential solution for decreasing energy usage and reducing carbon emissions.

While there are significant decarbonization benefits in electrification of residential heating, such a transition has important implications for gas and electric utilities.  From the perspective of a gas utility, as residential customers progressively switch from fossil-based heating to electric heat pumps, its customer base will shrink over time.  Since it incurs costs to maintain a gas distribution network which serves a dwindling customer base, a \emph{phased decommissioning} of its gas network becomes important -- switching entire neighborhoods to electric heating and shutting down the gas distribution in those neighborhoods.

Under this scenario, an electric utility will face the opposite problem -- as more homes switch to electrified heating, demand on the distribution grid will increase.  Upgrades may be required for electrical equipment (e.g. transformers) to address this demand.

Previous research efforts have studied decarbonization of heating and electrification from a homeowner's perspective, where homeowners are incentivized, based on their carbon emissions or carbon inefficiency, to convert to more efficient electric heat pumps.  However, such approaches encourage homeowners to make independent decisions which are agnostic of the gas network's topology or electric grid considerations.  While they reduce overall emissions, they may not enable gas utilities to reduce maintenance costs, especially if the electrified homes are scattered throughout a city and prevent the utility from reducing its distribution network.

A utility-based application where heat pump conversions are done in a planned manner, converting entire neighborhoods at a time, can yield significant benefits for both the gas and electric utilities -- the gas utility can shut down entire portions of its distribution network, reducing its maintenance burden, while the electric utility can address electrification via targeted grid infrastructure upgrades.

Such an approach requires a network-aware methodology which has access to the gas network's underlying topology.

In this paper, we....

In doing so, we make the following contributions.

==> oldsection3.tex <==
% \begin{itemize}
%     \item $t(j) = T_i$ -- transformer which serves $j$th house
%     \item $L(T_i)$ -- load profile for transformer $T_i$
%     \item $PL(T_i)$ -- peak load for transformer $T_i$
%     \item $c(T_i)$ -- capacity for transformer $T_i$
% \end{itemize}
% \noindent After gas lines are shut down and houses are chosen for conversion, we obtain a new load profile for all transformers in the network.  This can yield transformers which are \textit{newly overloaded} by the addition of electric heat pumps.  Formally, we have the following attributes:
% \begin{itemize}
%     \item $\mathcal{P}$ -- set of ``pruned'' (shutdown) gas lines
%     \item $\mathcal{O}$ -- set of newly overloaded transformers
%     \item $r_i$ -- cost to replace \& upgrade newly overloaded transformer $T_i$
% \end{itemize}

% \subsubsection{Edge Attributes}

% Each edge has:
% \begin{itemize}
%     \item gas line length (including connections to houses) $\leftrightarrow$ cost saved if shutdown
%     \item houses assigned to an edge \& their usage of gas
%     \item neighborhood location $\leftrightarrow$ equity
%     \item electric network connections for each house (transformer assignment)
% \end{itemize}

% \smallskip

% \noindent Each edge $(u, v) \in E$ has attributes associated with it:
% \begin{itemize}
%     \item $l_{u,v}$ -- total gas line length, which includes length of edge and house connections
%     \item $m(l_{u,v})$ -- maintenance cost for gas line (linear in length of the edge)
%     \item $\mathcal{H}_{u,v}$ -- set of houses assigned to $(u,v)$ 
%     \item $\mathcal{T}_{u,v}$ -- set of transformers serving households on $(u,v)$, including a mapping
% \end{itemize}

% \begin{itemize}
%     \item \; \pmb{+} \; conversion to electric heat pumps (per residence)\\
%     \item \; \pmb{+} \; Cost of necessary upgrades to the electric grid due to new heat pump load
%     \item \; \pmb{---} \; savings on maintenance cost due to gas shutdowns (per gas line edge)\\
% \end{itemize}
